Co-simulation of Continuous Systems: A Tutorial

Co-simulation consists of the theory and techniques to enable global simulation of a coupled system via the composition of simulators. Despite the large number of applications and growing interest in the challenges, the field remains fragmented into multiple application domains, with limited sharing of knowledge. This tutorial aims at introducing co-simulation of continuous systems, targeted at researchers new to the field.

==> fmi_standard.tex <==
\section{FMI Standard (Optional)}

This section goes over the FMI standard.

\claudio{There won't be time and space for this.}


==> notes.tex <==
\section{Planning}

\subsection{Random Thoughts}

Audience background is mostly computer science, but we assume that they know about differential equations.

We should have a complete running example, that can be incrementally built.
	The train and the person inside?
	 For completeness, we can have a person and a child. That will make the multi-rate part very interesting.
	Ideally, it should have scalar components, and then vector components.
	Ideally, it should be possible to highlights the flaws of co-simulation using that example.
  This example is nice because we can start with a cruise control system.
  And we can end with an exercise for the students (design a controller that is better than the one we provided)
  
  
Hans: We should not teach before differential equations.
We should show the equivalence between causal block diagrams and differential equations.

Describe differential equations (why, what and how)

Mention that we focus on diff equations, and explain why they are a general formalism. Link it to DAE's, to non-deterministic systems, etc\ldots
Mention how higher order diff equations can be mapped to this.

Describe co-simulation.
	Gauss seidel.
	Jacobi.
	Strong Coupling.

Give good introductory references for each of the topics. 
Instead of having inline citations in each section, maybe add a subsection on each concept explicitly saying where to get more information about those subjects.

Possible motivations for co-simulation: start with multi-rate; and having systems engineering.

\subsection{Concepts}

These are in progression of their complexity.

Extrapolation and Interpolation. Optional

Algebraic loops and fixed point iterations.

Integrals and Storage
	Great intuition about this in \cite[Chapter 2--3]{vanAmerongen2010}

Derivatives and Rates of Change.
	And our intuition about this.
	\cite[Section 2.7]{Stewart2008}
	\cite[Section 3.7]{Stewart2008}

Derivatives and Integrals -- Relationship and Intuitions
	Fundamental Theorem of Calculus		

Differential Equations
	Scalar differential equations
		How to model with scalar differential equations. Introduce the example.
		Explain the solution to differential equations.
		Explain how to transform the solution to a differential equation into a set of equations that when solved, give us an approximation of the differential equation.
			Analyze the solution procedure to those differential equations.
			Derive the forward euler method from there.
			Give the geometric intuition for the forward euler.
		Explain another way of approximating the solution to the differential equation (for backward euler). Optional
		\cite[Section 9.0]{Stewart2008}
	Vector differential equations
		Give the example of the mass spring damper.
		Show how the solution procedure is the same.

Co-simulation
	How do we arrive at co-simulation coming from the differential equations?
	We ways of motivating this separation: 
		Either have a control system that regulates stuff.
		Or have a subsystems which are of different orders of magnitude, and show the benefit of co-simulation.
			Multi-rate integration (\cite[Section 10.5]{Cellier2006})
			So the example has to have subsystems that are fast, and slow.
	Dimensions for the interfacing of different problems
		Gauss Seidel, Jacobi, Semi-explicit coupling, strong coupling.
		Iteration order (who goes forward first)
		Interpolation or Extrapolation
		Order of approximation methods
		Subsystem solver settings (e.g., mix of explicit and implicit method). This requires that backward euler is presented.
  










==> proposal.tex <==
\section{Proposal}

%%%%%% Summary 
\begin{comment}

Co-simulation consists of the theory and techniques to enable global simulation of a coupled system via the composition of simulators.
Each simulator is broadly defined as a black box capable of exhibiting behavior, consuming inputs and producing outputs.

This technique has been applied in a wide range of application domains.
However, due to its heterogeneous nature, there is limited sharing of findings between domains.

This tutorial is an attempt at facilitating the exchange of solutions and techniques, by promoting a deeper understanding of co-simulation.
To that end, we cover topics such as numerical approximation of differential equations and multi-rate integration, which can be seen as special cases of co-simulation.

Upon successful completion of this tutorial, the participants will have learned the necessary concepts to take their own routes in exploring this broad and fascinating field.

\end{comment}
%%%%%%

%%%%%% Why co-simulation is important.

Truly complex engineered systems that integrate physical, software and network aspects are emerging \cite{Nielsen2015}, posing challenges in their design, operation, and maintenance.

The design of such systems, due to market pressure, has to be concurrent and distributed, that is, divided between different teams and/or external suppliers, each in its own domain and each with its own tools.
Each participant develops a partial solution, that needs to be integrated with all the other partial solutions. 
The later in the process the integration is done, the higher its cost \cite{Plateaux2009}.
Ideally, the solutions developed independently should be integrated sooner and more frequently \cite{VanderAuweraer2013}.
%Furthermore, the traditional activities carried out at the partial solution level ---such as requirements compliance check, or design space exploration--- can be repeated at the global level, and salient properties spanning multiple constituent systems can be studied.

Modeling and simulation has improved the development of the partial solutions, but falls short in fostering this holistic development process \cite{Blochwitz2011}.
To understand why, one has to observe that:
\begin{inparaenum}[(i)]
\item models of each partial solution cannot be exchanged or integrated easily, because these are likely developed by a specialized tool;
\item externally supplied models may have Intellectual Property (IP) that cannot be cheaply disclosed to system integrators; and
\item as solutions are refined, the system should be evaluated by integrating physical prototypes, software components, and even human operators, in what are denoted as Model/Software/Hardware/Human-in-the-loop simulations \cite{AlvarezCabrera2011}.
\end{inparaenum}

Co-simulation consists of the theory and techniques to enable global simulation of a coupled system via the composition of simulators.
Each simulator is broadly defined as a \emph{black box} capable of exhibiting behaviour, consuming inputs and producing outputs.

%%%%%%


%%%%%% Why should we reinforce knowledge dissemination about it.

Despite the large number of applications and growing interest in the challenges that co-simulation poses (see, e.g., \cite{Gomes2017,Blochwitz2012}), the field is fragmented into multiple application domains, with limited sharing of knowledge.
To give an example, the use of dead-reckoning models is a well known technique in discrete event co-simulation \cite{Lee2000} and in adaptive control \cite{Garcia1989}, but only very recently it was used in a continuous time co-simulation approach \cite{Stettinger2014}.

%%%%%%

%%%%%% What knowledge are we going to focus on, and tutorial structure.

This tutorial aims at facilitating the exchange of solutions and techniques, by promoting a deeper understanding of co-simulation.
To that end, we assume minimal background on continuous systems modeling and simulation, and introduce the following topics:
\begin{compactenum}
%\item Derivatives and Integrals -- Relationship and Intuition
\item Differential Equations -- Scalar and Vector
\item Solution Approximation and Error -- The Forward Euler method
\item Decoupling Method -- Multi-rate integration
\item Generalized Decoupling Method -- Continuous time Co-simulation
\item The FMI Standard
\end{compactenum}
%The tutorial will make use of a single example, constructed as the topics are presented.
Further references, and a python notebook \footurl{http://jupyter.org/},  will be provided, so that participants can try the examples themselves, and build their own.
%A list of references is provided, in case participants want to know more.
%%%%%% 

%%%%%% What are the expected outcomes of the tutorial.
Upon successful completion of this tutorial, the participants will have learned the necessary concepts to take their own routes in exploring this broad and fascinating field.
%%%%%% 

